Sherlock: Scalable Fact Learning in Images

We study scalable and uniform understanding of facts in images. Existing visual recognition systems are typically modeled differently for each fact type such as objects, actions, and interactions. We propose a setting where all these facts can be modeled simultaneously with a capacity to understand unbounded number of facts in a structured way. The training data comes as structured facts in images, including (1) objects (e.g., $<$boy$>$), (2) attributes (e.g., $<$boy, tall$>$), (3) actions (e.g., $<$boy, playing$>$), and (4) interactions (e.g., $<$boy, riding, a horse $>$). Each fact has a semantic language view (e.g., $<$ boy, playing$>$) and a visual view (an image with this fact). We show that learning visual facts in a structured way enables not only a uniform but also generalizable visual understanding. We propose and investigate recent and strong approaches from the multiview learning literature and also introduce two learning representation models as potential baselines. We applied the investigated methods on several datasets that we augmented with structured facts and a large scale dataset of more than 202,000 facts and 814,000 images. Our experiments show the advantage of relating facts by the structure by the proposed models compared to the designed baselines on bidirectional fact retrieval.

==> sherlock_intro3.tex <==

\begin{comment}
\begin{quote}
\emph{I had come to an entirely erroneous conclusion, my dear Watson, how dangerous it always is to reason from insufficient data.}
~-Sherlock Holmes
\end{quote}
\end{comment}

\begin{comment}
\begin{quote}
\emph{It is a capital mistake to theorize in advance of the facts.}
~-Sherlock Holmes (The Adventure of the Second Stain)
\end{quote}
\vspace{-2mm}
\end{comment}

%\noindent\emph{It is a capital mistake to theorize in advance of the facts.}~-Sherlock Holmes~(\cite{DoyleSecondStrain})

The vast majority of the existing visual recognition methods assume a  fixed dictionary of visual facts. However, visual knowledge that we gain in our world is highly dynamic. Furthermore, different types of facts are modeled as different systems (e.g., different systems for object recognition, action recognition, interaction recognition, scene recognition, attribute recognition, etc).  A  human visual system is able to  efficiently  gain visual knowledge by learning facts of different types in a never ending process and from a few examples. Inspired by human visual perception, we present the problem of universal  visual recognition, where we propose one Language\&Vision approach that is able to learn objects, scenes, their attributes, their actions, and their interactions with other objects or scenes. Our fundamental \begin{wrapfigure}{r}{0.5\textwidth}   
  \vspace{-3mm}
   \includegraphics[width=0.5\textwidth]{knowledge_in_image.jpg}
       \vspace{-7mm}
    \caption{Sherlock Problem: Gaining Structured Visual Knowledge}
    \label{fig:imageknowledge}
    \vspace{-3mm}
\end{wrapfigure}idea for learning these facts together starts with introducing structure in their labels, categorizing labels into first order, second order and third order facts; see Fig.~\ref{fig:imageknowledge}. First Order Facts \textless S,*,*\textgreater\ are object categories and scenes (e.g., \textless baby\textgreater, \textless girl\textgreater, \textless beach\textgreater). Second Order Facts \textless S,P,*\textgreater\ are objects performing actions or attributed objects (e.g., \textless baby, smiling\textgreater, \textless baby, asian\textgreater). Third Order Facts \textless S,P,O\textgreater\ are interactions and positional information are represented by \textless S,P,O\textgreater\ (e.g. \textless baby, sitting\_on, high\_chair\textgreater, \textless person, riding, horse\textgreater ). Although it is common to label visual facts as only first order (e.g., \textless person\textgreater, \textless beach\textgreater), we argue that information in an image is usually more specific but we just label them in a limited way restricted to the task in hand. For example, we may find a \textless person, standing, *\textgreater ,  \textless person, leaning,* \textgreater , or \textless car, red, *\textgreater\  not just a person or a car. This motivates the structure we introduce to the label, where the S is the main subject of the fact and P is the attribute or action that modifies the appearance of S. In case of interaction, O represent the interacting object and P defines the interaction itself. Inspired from the concept of language modifiers, we then propose to model \textless S,P,*\textgreater\ and \textless S,P,O\textgreater\ facts as visual modifiers to \textless S,*,*\textgreater. For example, the second order fact \textless baby, smiling,* \textgreater\ is a visual modifier for \textless baby,*,*\textgreater, and the third order fact \textless person, playing, flute\textgreater\ is a visual modifier for both the second order fact \textless person, playing, *\textgreater\ and the first order fact \textless person\textgreater. We  argue that what makes recognition sometimes hard for some objects is the space of visual modifiers and how common it is, i.e., it might be easier to recognize a ``person'' modified by ``standing'' modifier \textless person, standing,*\textgreater\  (standing visual modifier)  compared to a person doing acrobatics \textless person, doing, acrobatics\textgreater. We think that the reason is that   some visual modifiers are  common (e.g., standing) and others are rare (e.g., doing acrobatics) during training, another view of the long-tail problem. An important observation is that the visual modifiers are more related to detailed appearance of an object like pose and color, which could be untangled in a visual recognition deep network and introduces a  need to be modeled by separate filters that we propose in this work; detailed in Model 2 in Sec.~\ref{sec_shmdls} . Hence, we propose to model universal visual  recognition along three continuous hyper-dimensions $\phi_S$, $\phi_P$, and $\phi_O$, where 
\begin{description}
\item [  $\phi_S \in \mathbb{R}^{d_S}$:] covers the space of object categories or scenes S. 

\item [  $\phi_P \in \mathbb{R}^{d_P}$: ]covers the space of actions, interactions, attributes, and positional information.
  
\item [    $\phi_O \in \mathbb{R}^{d_O}$:] covers the space of interacting objects, scenes that interact with S.
  \end{description}

For instance, first order facts like \textless girl,*,*\textgreater, \textless man,*,*\textgreater, \textless person,*,*\textgreater\   live in a hyper-plane in the $\phi_P \times \phi_O$ space; see Fig.~\ref{fig:vidmod}. Second order facts (e.g., \textless man, walking,*\textgreater, \textless girl, walking,*\textgreater) live as a hyper-line that is parallel to $\phi_O$ axis. Finally, a third order fact like \textless man, walking, dog\textgreater\ is a point in the  $\phi_S \times \phi_P \times \phi_O$ visual perception space. Meanwhile, this point lies on the \textless man, *, *\textgreater\  hyper-plane and the \textless man, walking, *\textgreater\ hyperline.  While we focus our experiments on \textless S,*,*\textgreater, \textless S,P,*\textgreater, \textless S,P,O\textgreater, our proposed setting assumes that there should be at least one non-wild card * in a training example including for example \textless *, walking, *\textgreater; see Fig~\ref{fig:vidmod}. We argue that modeling visual recognition based on this notion gives it a generalization capability since it allows us to learn facts like \textless man, *, *\textgreater, \textless girl, *, *\textgreater , \textless girl, walking, dog\textgreater\ during training, and it will be an expected behavior to be able to recognize \textless man, walking, dog\textgreater\ during testing even is never seen before. Another example is if a model learned the facts $<$boy, petting, a dog$>$, $<$girl,  riding, a horse$>$, and $<$boy$>$, it should be able to recognize an unseen fact $<$boy, petting, a horse$>$.  We observe this in our results in several unseen cases.% that came as a result from introducing this structure.  





 
\begin{figure}[t!]
    \vspace{-13mm}
  \centering
    \includegraphics[width=0.9\textwidth]{vis_modifier_fig.jpg}
      \vspace{-4mm}
    \caption{Visual Modifiers Notion}
    \label{fig:vidmod}
        \vspace{-6mm}
\end{figure}






We model structured knowledge in images as a problem that comes with two views, one in the visual domain $\mathcal{V}$ and one in the language domain $\mathcal{L}$. 
%We start by introducing some notation. 
Let $\mathbf{f}$ be a structured fact,  $\mathbf{f}_v \in \mathcal{V}$ denoting the view   of $\mathbf{f}$ in the visual domain and $\mathbf{f}_l \in \mathcal{L}$ denoting the view of $\mathbf{f}$ in the language domain. For instance, an annotated fact with language view $\mathbf{f}_l = <$S:girl, P:riding, O:bike$>$ would have a corresponding visual view $\mathbf{f}_v$ as an image where this fact occurs; see Fig.~\ref{fig:probdef}.

\begin{comment}
\begin{figure}[t!]
  \centering
    %\includegraphics[width=0.5\textwidth]{sherlock_problem_def.png}
    \includegraphics[width=0.39\textwidth]{sherlock_problem_def_new.jpg}
    \caption{Problem Definition}
    \label{fig:probdef}
    \vspace{-10mm}
\end{figure}
\end{comment}

%{sherlock_problem_def_new.jpg}
Our goal is to learn a representation that covers  first-order facts $<$S,*,*$>$ (objects), second-order facts $<$S,P,*$>$ (actions and attributes), and third-order facts $<$S,P,O$>$ (interaction \begin{wrapfigure}{r}{0.5\textwidth}   
\centering
  \vspace{-5mm}
    \includegraphics[width=0.5\textwidth,height=0.35\textwidth]{problem2.png}
      \vspace{-6mm}
    \caption{Problem Definition}
      \vspace{-7mm}
    \label{fig:probdef}
    \vspace{-6mm}
\end{wrapfigure}and positional facts). We represent all types of facts as an embedding problem into  what we call ``structured fact space''. We define ``structured fact space'' as a learning representation of the  $\phi_S \in \mathbb{R}^{d_S}$, $\phi_P \in \mathbb{R}^{d_P}$, and $\phi_O \in \mathbb{R}^{d_O}$  hyper-dimensions (Fig.~\ref{fig:probdef}). We denote the embedding functions  from a visual view of a fact  $\mathbf{f}_v$ to  $\phi_S$, $\phi_P$, and $\phi_O$ as  $\phi^{\mathcal{V}}_S(\mathbf{f}_v)$, $\phi^{\mathcal{V}}_P(\mathbf{f}_v)$, and $\phi^{\mathcal{V}}_O(\mathbf{f}_v)$, respectively. Similarly, we  denote the embedding functions from a language view of a fact  $\mathbf{f}_l$ to  $\phi_S$, $\phi_P$, and $\phi_O$ as  $\phi^{\mathcal{L}}_S(\mathbf{f}_l)$, $\phi^{\mathcal{L}}_P(\mathbf{f}_l)$, and $\phi^{\mathcal{L}}_O(\mathbf{f}_l)$, respectively. We denote the concatenation of the visual view  hyper-dimensions' embedding as $\phi^{\mathcal{V}}(\mathbf{f}_v)$, and the language view   hyper-dimensions' embedding  as $\phi^{\mathcal{L}}(\mathbf{f}_l)$, where  $\phi^{\mathcal{V}}(\mathbf{f}_v)$ and  $\phi^{\mathcal{L}}(\mathbf{f}_l)$ are  visual embedding and language embedding of $\mathbf{f}$, respectively:
\begin{equation}
\begin{split}
\phi^{\mathcal{V}}(\mathbf{f}_v) = [\phi^{\mathcal{V}}_S(\mathbf{f}_v), \phi^{\mathcal{V}}_P(\mathbf{f}_v),  \phi^{\mathcal{V}}_O(\mathbf{f}_v) ], 
\phi^{\mathcal{L}}(\mathbf{f}_l) = [\phi^{\mathcal{L}}_S(\mathbf{f}_l), \phi^{\mathcal{L}}_P(\mathbf{f}_l), \phi^{\mathcal{L}}_O(\mathbf{f}_l)]
\end{split}
\label{eq1}
\end{equation}
% $\phi^{\mathcal{V}}_S(\mathbf{f}_v)$, $\phi^{\mathcal{V}}_P(\mathbf{f}_v)$, and $\phi^{\mathcal{V}}_O(\mathbf{f}_v)$as $\phi^{\mathcal{V}}(\mathbf{f}_v)$ = [$\phi^{\mathcal{V}}_S(\mathbf{f}_v)$, $\phi^{\mathcal{V}}_P(\mathbf{f}_v)$,  $\phi^{\mathcal{V}}_O(\mathbf{f}_v)$ ]. Similarly, we denote the concatenation of $\phi^{\mathcal{L}}_S(\mathbf{f}_l)$, $\phi^{\mathcal{L}}_P(\mathbf{f}_l)$, and $\phi^{\mathcal{L}}_O(\mathbf{f}_l)$ as $\phi^{\mathcal{L}}(\mathbf{f}_l)$ = [$\phi^{\mathcal{L}}_S(\mathbf{f}_l)$, $\phi^{\mathcal{L}}_P(\mathbf{f}_l)$,  $\phi^{\mathcal{L}}_O(\mathbf{f}_l)$]. 

%This opens the question of what is a training example in Universal visual recognition. 
%\ignore{ For example if during training a model learned the facts $<$boy, petting, a dog$>$, $<$girl,  riding, a horse$>$, and $<$boy$>$, it should be able to recognize an unseen fact fact $<$boy, petting, a horse$>$ even though it did not see that fact before}

 \textit{Modeling the connection  between the provided structured facts in its language form and its visual view 
%(i.e., an image containing it) 
facilitates  gaining richer visual knowledge, which is our focus in this paper}. We further show that modeling universal visual perception as a Language\&Vision problem have several advantages: (1)  \textbf{highly dynamic}: can be given fact language-visual view pairs in a never ending way to gain more structured knowledge. (2) \textbf{generalization}: could generalize to unseen facts. (3) \textbf{bi-directional}:  allows retrieval of both the fact language view given the visual view and vice versa.    (4) \textbf{wild-cards}: In order to model different types of facts in one model, we present the notion of visual modifiers, where higher order facts (e.g., \textless baby, smiling,*\textgreater) are modeled as visual modifiers of lower order facts. We train using a novel wild-card loss function which allows learning all different types of facts in one model, detailed in Sec.~\ref{sec_shmdls}. Since the proposed setting is aiming for a model that has an eye for details and potentially allows higher order reasoning (Fig.~\ref{fig:imageknowledge}), we denote this problem as the Sherlock Problem.   %Since this is a new setting, we present the first dataset on this task that consists of 800,000 images and 202,000 structured facts of different types. A big part of this data was collected by a method that (2) able to learn a representation which  covers different types of structured facts,  , (, and

  %Several applications can make use of more thorough and structured information captured from an image, such as  structured fact tagging, high precision image search from text, generating comprehensive descriptions of complicated scenes, and making higher level reasoning about a scene. 
%Like a good detective, we are interested in determining a set of facts about an image, such as what objects are present, what are they doing, and how they interacting with each other, by modeling the knowledge in an image.  Modeling knowledge in images makes the connection between language and vision more inherent and explicit. 

\textbf{Data Collection in our setting:} This is a new setting and in order to train a model for our setting, we needed to collect structured fact annotations in the form of (language view, visual view) pairs (e.g.,  $<$baby, sitting on, chair$>$ as the language view and an image with this fact as a visual view). This is a challenging task. We started by manually annotating and mining several existing datasets to extract structured fact annotations, which we found limiting for both the dataset size and for covering different types of facts  (Sec.~\ref{sec_data}). One of the most interesting relevant works is the Never Ending Image Learner (NEIL)~\citep{chen2013neil}, where they showed that  visual concepts predefined in an ontology can be learnt by collecting its training data from the web. In a  follow-up work,~\cite{divvala2014learning} collected images from the web for concepts related to a predefined object using Google-N-gram data. This opens the question of whether we can collect structured fact annotations from the web. There are two issues we face in our setting. 
First, it is difficult to define the space of structured visual knowledge and then search for it. Second, using Google image search is not reliable to collect data for concepts with fewer images on the web. The main assumption for this method  depends on both the likelihood that the top retrieved image belongs to the searched concept, and the availability of  images annotated with the searched concept. These problems motivated us to propose a novel method to automatically annotate structured facts  by  processing image caption data since structured facts in image captions are highly likely to be located in the image.
%Our Sherlock Automatic Fact Annotation (SAFA) starts by processing challenging unconstrained noisy captions to extract fact language view by multiple methods. 
Our Sherlock Automatic Fact Annotation (SAFA) method extracts fact language views from image captions and then localizes the facts to image regions to get visual views.   
%Then we ground the  facts extracted from captions to image regions to get visual views.   
%There are two advantages of collecting structured fact annotations by the proposed method. First,  it assumes that structured facts in the captions are likely to be located in the given image, which is expected to occur in image-caption data with a very high probability compared to the assumptions in~\citep{chen2013neil,divvala2014learning} and  makes it likely to produce accurate annotations as we show in our results. Second,  it could be used to collect knowledge very cheaply for several tasks. Our automatic annotations resulted in hundreds of thousands of images and tens of thousands of unique  knowledge annotations 
%%, needed to feed our  model, 
%in just several hours with our current implementation.
%% whose speed is far from optimal
SAFA collected tens of thousands of unique knowledge annotations within hundreds of thousands of images in just several hours. 


\textbf{Contributions. }There are three main contributions in this paper: (1) We introduce the Sherlock problem of modeling universal visual recognition and propose the visual modifiers notion that enables learning structured facts of different types  and performs both-view retrieval (retrieve structured fact language view (e.g. $<$S:people, P:walking$>$) given the visual view (i.e. image) and vice versa).
(2) We propose an automatic stuctured fact annotation method based on sophisticated Natural Language Processing methods for acquiring high quality structured fact annotation pairs at large scale from free-form image descriptions. We applied the pipeline to MS~COCO~\cite{lin2014microsoft} and Flickr30K~Entities~\cite{plummer2015flickr30k,young2014image} image caption datasets. In total, we build a structured fact dataset of more than $816,000$ language\&image-view fact pairs covering more than $202,000$ unique facts in the language view. 
(3) We develop a novel learning representation network architecture to jointly model the structured fact language and visual views  by mapping both views into a common space and using a wild card loss to uniformly represent first, second, and third order facts. Our modeling approach is scalable to new facts without any change to the network architecture.


%We consider the problem of gaining visual knowledge in a never ending process, where knowledge is defined by a set of visual facts without any restriction. In our setting facts reaches hundreds of thousands. We start by defining a visual fact. 

%\textbf{Facts in image: } Facts that one might learn from an image include objects, scenes,  attributed objects (e.g., ``red car''), objects performing an action (e.g., ``person jumping''), interaction (e.g., ``person riding horse''). Our goal is to modeling gaining visual knowledge by learning facts with generalization capabilities and with wild-card access.







%\textbf{Goal:} Our goal is to propose a well-motivated 

%We hypothesize that a fact in an image is usually more specific, but they are mainly abstracted category labels for action recognition, action labels for activity recognition, attribute labels for attribute recognition. 
%We propose to model visual recognition as a multi-view problem.  learning $\psi: \mathcal{V} \times \mathcal{L} \to \mathbb{R}$. 
 %Recognition  might include actions, attributes and interactions, which have been studied as different tasks~\citep{}


%Visual recognition tasks has been mainly studied separately 

%Several methods has been proposed to learn visual classifiers for several visual recognition tasks, which is commonly addressed as a mapping function 


















%In our work, we aim to cover three types of facts by the same model. First order facts in images are defined by the set of objects and the scene in an image (e.g,. $<$baby$>$, $<$toy$>$, $<$bathroom$>$). Second order facts are defined by attributes and single-frame action that might be performed by the objects (e.g., $<$ baby, smiling$>$, $<$man, dancing$>$). An object interacting with another object defines a third order fact in the image (e.g., $<$man, feeding, baby$>$,  $<$baby, sitting on, chair$>$).  We denote the first, second, and third order facts by $<$Subject$>$, $<$Subject, Predicate$>$, and $<$Subject, Predicate, Object$>$  respectively, abbreviated as  $<$S$>$, $<$S,P$>$, and $<$S,P,O$>$; see Fig.~\ref{fig:imageknowledge}. Inspired by the modifier concept in language grammar, we model higher order  facts as visual modifiers of the low order facts. For example, $<$baby, smiling$>$ is applying the $<$smiling$>$ visual modifier to $<$baby$>$. Based on this notion,  we propose a model for learning a representation of structured facts covering different orders that can be continuously fed with these facts to gain structured knowledge.
%\begin{comment}
%\end{comment}
%Specifically, both language and visual views of a structured fact inhabit in a continuous space.  Modeling structured facts in a continuous space  allows us to extend the gained knowledge from the training facts to unseen facts. For example if during training a model learned the facts $<$boy, petting, a dog$>$, $<$girl,  riding, a horse$>$, and $<$boy$>$, it should be able to recognize the fact $<$boy, petting, a horse$>$ even though it did not see that fact before.  Since the proposed setting is aiming for a model that has an eye for details and potentially allows higher order reasoning (Fig.~\ref{fig:imageknowledge}), we denote this problem as the Sherlock Problem. 

%Looking at an image, there are typically a lot of "facts'' that we can extract. For example in Figure~\ref{fig:imageknowledge}, there are several facts such as "man is feeding the baby'', "the man is smiling", "baby is smiling", "baby is holding a toy'', etc..  Connecting this  structured representation of facts in an image to State-of-the-art captioning methods (e.g., ~\cite{karpathy2014deep,vinyals2015show,xu2015show,mao2015deep}), one might argue that while captioning systems are impressive step towards enabling    %Our goal is to build a system that can generate many of these facts about a given image.



%Connecting language and vision has been a topic of great interest in the last few years.   rely on the idea of generating a sequence of words given an image of a scene.  However, captioning systems are incapable of conveying structured information that might appear in the scene and providing a confidence of the generated caption given the facts that appear in the scene.  They also may miss many interesting objects and actions in the scene.  



\begin{comment}
Many computer vision researchers produce a tremendous amount of work to improve computer vision as a detective eye for machines. 
There is a whole spectrum of ways to render exracted knowledge from images. 
Traditionally, object, scene, and activity categories are reported. Image tagging approaches aim at representing multiple object and scene categories, and probably attributes for a given images. To the other end, image captioning system aim at rendering full sentences describing the content in the image.
\end{comment}




% Image tagging approaches aim at representing multiple object and scene categories, and probably attributes for a given images. 

%\begin{figure}[htb!]
%\begin{figure}[t]
%  \centering
%    \includegraphics[width=0.45\textwidth]{knowledge_in_image.png}
%    \caption{Structured Knowledge in an Image}
%    \label{fig:imageknowledge}
%    \vspace{-8mm}
%\end{figure}


%Besides scalability, the machine has to be able to generalize to recognize unseen facts. For example if we learn during training about ``girl smiling'', ``boy petting a dog'', ``girl riding a horse'', and ``boy'', the system should be able to recognize the fact ``boy petting a horse'' even though it did not see that fact before. 



%In order to achieve the aforementioned qualities, we define three types of facts in images (see Fig.~\ref{fig:imageknowledge}).  

 %As a result, the model can generate several structured facts for a given test image encoding the rich information in the image.  

%\textbf{{How can we collect structured fact annotations needed to train a Sherlock Model?}}


%The grounding process  involves word sense disambiguation~\cite{zhong2010makes}, wordNet ontology~\cite{leacock1998combining}.

%In order to learn the model, we needed to collect data of fact-image pairs where facts comes in structured form (i.e.,  $<$baby, sitting on, chair$>$ ), which is a challenging problem. Our data collection efforts started by annotating the fact language view  of six existing datasets, detailed later. However, this limited us to only ~28K images and 186 unique facts.  We propose a framework for automatically annotating knowledge in images by developing a method that can process images with captions and extract structured annotation and further localize them in images. Our Sherlock Automatic Fact Annotation (SAFA) started by processing challenging unconstrained noisy captions to extract knowledge by multiple methods. Then, we grounded the extracted knowledge from captions to image regions involving word sense disambiguation, wordNet ontology.  This pipeline could be used to collect knowledge very cheaply for several tasks. Our automatic annotations resulted in hundreds of thousands of images and tens of thousands of unique  knowledge annotations, needed to feed our proposed deep model. 

\begin{comment}
Connecting language and vision has been a topic of great interest in the last few years.  State of the art captioning methods (e.g., ~\cite{karpathy2014deep,vinyals2015show,xu2015show,mao2015deep}) rely on the idea of generating a sequence of words given the whole image as a scene, and several new benchmarks have been proposed for this task (e.g, MS COCO dataset~\cite{lin2014microsoft}, Flickkr30K(~\cite{young2014image}).  However, state-of-the-art captioning systems are incapable of conveying structured information that might appear in the scene and providing a confidence of the generated caption given the correct facts that appears in the scene.  They also may miss many interesting objects and actions in the scene. 
\end{comment} 

\begin{comment}
After all, captions are mainly a vehicle to communicate knowledge with humans, however, they might not be the best way to represent that knowledge in a way that is  searchable for the machine. Therefore, in this paper we focus on generating structured facts from images. Many applications can make use of structured information captured from the whole image, such as  structured knowledge tagging, knowledge extraction from image, high precision image search from text, generating captions of complicated scenes, and image knowledge abstraction.
\end{comment}

\begin{comment}
The contributions of this paper are as follows:


\vspace{-2mm}
\begin{itemize}[leftmargin=*]
\item Build a joint probabilistic model P($<$S,P$>$ , Image, I), P($<$S,P,O$>$, Image, I) to output the probability that image I and structured text $<$S,P$>$ or $<$S,P,O$>$ represent the same real world concept visually and textually. The proposed model generalizes well to unseen or rarely seen combinations of subjects, attributes, predicates, and objects. The model does not require explicitly reducing from a large vocabulary of individual words to a small, pre-defined set of concepts.
\item Automatically compute a representation of an image as a set of structured, semantic knowledge in the form of a knowledge tuples that describe the objects and their interactions in the input image and that are localized within the image.
\item  Use Natural Language Processing (NLP) methods for automatic semantic knowledge extraction from free-form (unstructured) text associated with images to collect a large training dataset of knowledge tuples.
\end{itemize}
\end{comment}

 \vspace{-1mm}

%The contributions of this paper are as follows:


\begin{comment}
\vspace{-3mm}
\begin{itemize}
\setlength{\itemsep}{1pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
\item We introduce the Sherlock problem of structured knowledge modeling in an image and propose a model that can learn structured facts of different types  and perform both-view retrieval (retrieve structured fact language view (e.g. $<$S:people, P:walking$>$) given the visual view (i.e. image) and vice versa.
\item We propose an automatic stuctured fact annotation method based on sophisticated Natural Language Processing methods for acquiring high quality structured fact annotation pairs at large scale from free-form image descriptions. We applied the pipeline to MS~COCO~\cite{lin2014microsoft} and Flickr30K~Entities~\cite{plummer2015flickr30k,young2014image} image caption datasets. In total, we build a structured fact dataset of more than $816,000$ language\&image-view fact pairs covering more than $202,000$ unique facts in the language view. 
\item We develop a novel learning representation network architecture to jointly model the structured fact language and visual views  by mapping both views into a common space and using a wild card loss to uniformly represent first, second, and third order facts. 
\end{itemize}
\vspace{-2mm}
\end{comment}

%, and our automated pipeline for creating training data from free-form image descriptions can be used to efficiently feed new data into the model in the future.

%We suggest a method for automatically extracting a set of relevant facts for a given image area (and therefore for an entire image by repeated application).
%(2) automatic pipeline for acquiring training data (including grounding) at scale from unstructured image annotations for a machine learning approach to this problem (and the training data is potentially useful for other problems/applications).
%(2.5) We release our large dataset of (fact,image) pairs?! Depends on how good it is?
%(3) Our common space deep network for jointly modeling (fact,image) with separate tuning filters for subjects and for (predicate,object pairs), viewing predicates and objects as visual modifiers of subjects, and wild card loss to uniformly represent first, second, and third order facts. 
%Our modeling approach is scalable and enables use of easily obtainable training data.
%\item We introduce the Sherlock problem of structured knowledge modeling in an image. 
%\item We propose to leverage existing image caption datasets and other data sources with free form image descriptions to collect (structured knowledge, image region) pairs for machine learning approaches to this problem.
%\item We provide an automatic method for extracting the best structured facts for a given image region (knowledge extraction or {\em structured tagging}) and the best images for a given structured fact (image retrieval).  
%\item We propose an automatic pipeline based on sophisticated Natural Language Processing methods for acquiring high quality (structured knowledge, image region) training data at large scale from free form (unstructured) image descriptions. 


==> sherlock_relwork.tex <==
In order to make the contrast against related work clear, we start by stating the scale of facts we are modeling in this work. Let's assume that $|$S$|$, $|$P$|$, and $|$O$|$ denotes the number of  unique subjects, unique predicates, and unique objects, respectively.  The scale of unique second and third order facts is bounded by $|$S$|\times |$P$|$ and  $|$S$| \times |$P$| \times |$O$|$ possibilities respectively,  which can easily reach millions of unique facts and needs careful attention while designing a model maintaining the structure we aim at.  The data we collected in this work has thus far reached 202,000 unique facts (814,000 images).%, which continue to grow. 
%The scale of unique second and third order facts could easily reach millions of unique facts and needs careful attention while designing a model maintaining the structure.


\textbf{(A) Modeling Visual facts in Discrete Space: }
Visual Recognition tasks like object or activity recognition have been typically addressed  as a mapping function $g: \mathcal{V} \to \cal{Y}$, where $\cal{Y}$ is discrete set of classes $1 \to K$. The function $g$ was traditionally learned over engineered features like variants of SIFT features (e.g.,~\cite{bosch2007image}), and  have recently been learned using deep learning (e.g.,~\cite{simonyan2014very,Szegedy_2015_CVPR}. Nowadays, different methods/systems are built to recognize facts in images by modeling  a different $g: \mathcal{V} \to \cal{Y}$ , where $\cal{Y}$ is constrained to certain facts for each approach. Examples of different  $\cal{Y}$ for different facts include (1) object categories, (e.g.,~\cite{simonyan2014very}),  (2) attributes (e.g.~\cite{zhang2014panda}), (2) attributed objects $<car, red>$~\cite{chen2014inferring}, (3) scenes (e.g., ~\cite{zhou2014learning}), (4) activities  (e.g.,~\cite{gkioxari2014finding}, and (5) interactions~\cite{Antol2014}. This opens the question of why we build different systems or approaches for these related tasks since images usually contain objects with particular attributes performing an action or interacting with another object. We think that there are several limitations in modeling visual recognition as $g: \mathcal{V} \to \cal{Y}$. \textbf{(1)} Grouping visual facts and modeling each group by a different $g$, while a human visual perception system is able to incrementally learn visual facts (objects, interactions, actions, attributes classes, etc) as one system. In the real world, this means that we need to group each visual fact type in order to deal with a different recognition system for each group and then retrain several models. \textbf{(2)} Adding a new fact leads to changing the architecture, meaning adding thousands of parameters 
and re-training the model (e.g., needed for adding a new output node). If we used VGGNet for instance on the scale of 202K facts, the number of parameters in the softmax layer alone gets very close to 1 billion parameters. GPU memory does not fit this number of parameters and makes learning a big challenge. \textbf{(3)} While the majority of the existing benchmarks have at least tens of examples per fact (e.g., imageNet~\citep{deng2009imagenet}),  a more realistic assumption for visual recognition is  that there might not be enough examples for the newly added examples to learn the new class, which introduces a learning problem. This problem is know as the long-tail,   where several works have been proposed to deal with in the object recognition setting following a ditribution similar to Zipf's law ~\citep{zipf1935psycho,salakhutdinov2011learning}.\textbf{(4)} These models are only uni-directional from $\cal{V}$ to $\cal{Y}$.


%Based in the most recent imageNet challenge results in object recognition, several researchers argue that the visual recognition problem is solved. Even though object recognition performance is rapidly reaching maturity, this does not mean that existing machine learning methods is able to recognize complex facts in the visual world. 


%There are indeed other research problems that aim to explicitly understand facts about an image.
%The main objective in object (e.g.,~\cite{simonyan2014very}), scene (e.g., ~\cite{zhou2014learning}), and activity categorization (e.g.,~\cite{gkioxari2014finding}) methods is to have a set of discrete categories that the system can recognize.  These methods face  a scalability problem since adding a new category means changing the architecture 
%of the model by adding thousands of parameters 
%and re-training the model (e.g., needed for adding a new output node). This drawback is also shared with recent attribute based methods (e.g., ~\cite{chen2014inferring}) that realize that attribute appearance is dependent on the class,  unlike earlier models (e.g.,~\cite{lampert2009learning}).  
%This motivates them to jointly learn a classifier for every class attribute pair, which suffers from  scalability problems  as the number of the classes and attributes grows.  Our goal is to model structured facts in a way that is scalable, i.e., to avoid the need to change the model in order to add more facts. Furthermore, we aim that the model can gain structured visual knowledge by being continuously fed with instances of structured  facts,  that could be of different types (e.g.,  $<$woman,  smiling$>$, or $<$person, playing, soccer$>$, $<$ man, tall$>$, $<$kid$>$) with example image(s). At any point the machine does not have a fixed dictionary of trained object, scene, activity categories.



\textbf{(B)  Modeling zero/few shot fact learning by attributes: } One of the most successful ideas for learning from few examples per class is by using semantic output codes or attributes as an intermediate layer between features and class. Formally,  $g$ is composition of two function $g={h}({a}(\cdot))$, where $a: \cal{V} \to \cal{A}$, and $h: \cal{A} \to \cal{Y}$~\citep{palatucci2009zero}. The main idea is to collect data that is sufficient to learn about the intermediate attribute layer, where classes are then represented by these attributes to faciltate zero-shot/few-shot learning. However,  ~\cite{chen2014inferring} realize that attribute appearance is dependent on the class,  as opposed to these earlier models~\citep{palatucci2009zero,lampert2009learning}. Although~\cite{chen2014inferring}'s assumption is more realistic, learning different classifiers for each category-attribute pair introduces the scalability and learning difficulties pointed out in (A), limits the model's applicability, and still restricts the model to certain groups of facts. In contrast, our goal is a method that can learn any visual fact in an incremental way. It is worth mentioning that there is a huge body of work in incremental learning (e.g.~\cite{Bendale_2015_CVPR}), but it mainly focuses on the object recognition task and assumes   labels $\cal{Y}$ lives in a  discrete space (not tractable for universal visual recognition).   Furthermore ~\cite{Bendale_2015_CVPR} also assumes that each image has only one fact, which is not a  restriction in our work (e.g., same image could have \textless person, *,*\textgreater\ and \textless man,  jumping\textgreater). Also, the notion of similar classes is not addressed in the vast majority of these works. For instance, \textless person, *,*\textgreater\ is expected to be more similar to \textless man, *,*\textgreater\ than to \textless fish, *,*\textgreater, which makes a stronger motivation for learning facts in a continuous space.  

%Our goal is to model visual recognition universally that shows a better generalization capability and in a  never-ending process, such that one model can learn get continuously fed with facts and learn new visual facts similar to human.



%Some researchers may hypothesize that the visual recognition problem is reaching a solved  state, given the rapid progress in this problem. However,  there are several aspects of visual recognition that goes beyond that object recognition tasks like imageNet~\cite{deng2009imagenet}.  




 %From this point, we might refer to a structured fact as simply a fact for simplicity.   %Still the machine should be able to generate multiple of these structured facts about a test image. 

%Sharing attributes between classes as an intermediate layer has been shown to be effective for categorization, zero shot learning and few shot learning~\cite{lampert2009learning,lampert2014attribute}. However, the main assumption behind existing methods is that classes are independent of the image given the attributes and hence attributes are independent of the attributes. More recent work~\cite{chen2014inferring} realizes the idea that attribute appearance is dependent on the class,  which motivates them to jointly learn a classifiers for every class attribute pair, which clearly have a scalability problems and the number of the classes and attributes grows.  The problem is further complicated when building a model to learn high order knowledge in images (first, second and third order).   By jointly modeling images and knowledge in continuous space, we can handle this higher order knowledge by having similar concepts have nearby and related representations.

\textbf{(C) Object Recognition in continuous space using Vision and Language:}
Recent works in language and vision involve using  unannotated text to improve object recognition and to achieve zero-shot learning. The following group of  approaches model object recognition as a function 
%$g: {\arg\max}_y\,\, s(v \in \cal{V} ,$ $y  \in \cal{Y})\to \mathbb{R})$, 
$g(v) = {\arg\max}_y\,\, s(v \in \cal{V} ,$ $y  \in \cal{Y})$, 
where $s(\cdot,\cdot)$ is a similarity function between image $v$ and class $y$ represented by text.   
In~\citep{NIPS13DeViSE},~\citep{norouzi2014zero} and~\cite{NIPS13CMT},  word  embedding language models (e.g.,~\cite{mikolov2013distributed}) were adopted to represent class names as vectors.  Their framework maps images into the learned language model and then does classification in that space. In addition to that our setting is different,   imageNet dataset in their case has 1000 object facts with thousands of examples per class. Our setting has two orders of magnitude more facts with long-tail distribution. Conversely, other works model the mapping of unstructured text descriptions for classes  into a visual classifier~\citep{elhoseiny2013write,ba2015predicting}. %In contrast, our goal is to gain visual knowledge for not only  first order facts $<$S$>$ but also for second  $<$S$,$P$>$, and third order facts $<$S$,$P$,$O$>$, and also maintain the structure of the facts. 
We are extending the visual recognition task to the scale of millions of facts, not only object recognition but also understanding their attributes, actions, and interactions in one model. Our labels are also structured, where we handle missing parts like P and O in  \textless dolphin, *,*\textgreater\ examples and O in  \textless girl, playing,*\textgreater, which enables our method to learn facts of different types by the wild-card loss we introduce. Furthermore, we propose the visual modifiers notion, which motivates us to learn separate branches of convolutional filters that outperforms more straightforward convolutional baselines that we designed for this task; see Sec~\ref{sec_shmdls}. 

%Let's assume that $|$S$|$, $|$P$|$, and $|$O$|$ denotes the number of  subjects, predicates, and objects, respectively.  
%The scale of unique second and third order facts is bounded by $|$S$|\times |$P$|$, and  $|$S$| \times |$P$| \times |$O$|$ possibilities respectively that could easily reach millions of unique facts and needs careful attention while designing a model maintaining the structure. %we aim at.  
%The scale of unique second and third order facts could easily reach millions of unique facts and needs careful attention while designing a model maintaining the structure.

%however, they suffer from the 
%aforementioned 
%scalability limitation. % Do we need to argue about \cite{sadeghi2015viske}







